MobiGuide: Vocabulary-Guided Online Recovery for Mobile Manipulation

A central challenge in mobile manipulation is preserving multiple plausible action modes while remaining reactive during execution. For example, grasping a bottle in a cluttered scene can be achieved through multiple physically feasible base-arm motion plans. Deterministic VLA policies trained with $L_1$ regression are efficient, but they tend to average across valid modes and may produce physically invalid actions. Diffusion-based generative policies can better represent multimodal action distributions, yet their proposals may be weakly constrained when generated from pure noise, and iterative sampling can increase inference cost. Action chunking helps amortize inference, but it also introduces partially open-loop execution, allowing small mismatches to accumulate into drift. We present MobiGuide, a generative VLA model for efficient mobile manipulation, where action generation is guided by a structured trajectory vocabulary. Constructed from expert demonstrations, this vocabulary encodes plausible whole-body motion patterns and provides structured priors for feasible action generation. Given the current observation and instruction, MobiGuide locally refines these reference trajectories into context-compatible action proposals and selects the most suitable trajectory for execution. This preserves multimodal action candidates while keeping generation constrained around feasible expert-like motion modes. To mitigate chunk-induced drift, we further introduce a lightweight residual correction module that performs high-frequency, per-step adjustments during rollout. Across diverse mobile manipulation tasks, MobiGuide improves success and stability under execution disturbances while maintaining low-latency inference.

==> references_compact_setup.tex <==
% Load this file in your existing manuscript PREAMBLE:
%   \input{references_compact_setup}
% Keep your conference document class, font sizes, margins and spacing unchanged.
%
% At the existing bibliography location, use:
%   \bibliographystyle{IEEEtran}
%   \bibliography{references_compact}
%
% This setup is for BibTeX + IEEEtran.bst, not biblatex/Biber.
\usepackage{url}

% IEEEtran.cls supplies \bstctlcite. Other classes (such as ieeeconf)
% can obtain it from IEEEtrantools without changing the document class.
\makeatletter
\@ifundefined{bstctlcite}{\RequirePackage{IEEEtrantools}}{}
\makeatother

% Process the formatting-control entry before ordinary in-text citations.
% Unlike \nocite, \bstctlcite does not require a numbered bibliography item.
\AtBeginDocument{\bstctlcite{compactrefs}}

